Controlling an Inverted Pendulum with Policy Gradient Methods-A Tutorial

This paper provides the details of implementing two important policy gradient methods to solve the inverted pendulum problem. These are namely the Deep Deterministic Policy Gradient (DDPG) and the Proximal Policy Optimization (PPO) algorithm. The problem is solved by using an actor-critic model where an actor-network is used to learn the policy function and a critic network is to evaluate the actor-network by learning to estimate the Q function. Apart from briefly explaining the mathematics behind these two algorithms, the details of python implementation are provided which helps in demystifying the underlying complexity of the algorithm. In the process, the readers will be introduced to OpenAI/Gym, Tensorflow 2.x and Keras utilities used for implementing the above concepts.

==> pygtex_files/actor_model-py.tex <==
\begin{Verbatim}[commandchars=\\\{\},baselinestretch=0.9,frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\tiny]
\PY{k}{class} \PY{n+nc}{PPOActor}\PY{p}{:}
    \PY{k}{def} \PY{n+nf}{\PYZus{}build\PYZus{}net}\PY{p}{(}\PY{n+nb+bp}{self}\PY{p}{)}\PY{p}{:}
        \PY{n}{last\PYZus{}init} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{random\PYZus{}uniform\PYZus{}initializer}\PY{p}{(}\PY{n}{minval}\PY{o}{=}\PY{o}{\PYZhy{}}\PY{l+m+mf}{0.003}\PY{p}{,} \PY{n}{maxval}\PY{o}{=}\PY{l+m+mf}{0.003}\PY{p}{)}
        \PY{n}{state\PYZus{}input} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Input}\PY{p}{(}\PY{n}{shape}\PY{o}{=}\PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{state\PYZus{}size}\PY{p}{)}
        \PY{n}{l} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Dense}\PY{p}{(}\PY{l+m+mi}{128}\PY{p}{,} \PY{n}{activation}\PY{o}{=}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{relu}\PY{l+s+s1}{\PYZsq{}}\PY{p}{)}\PY{p}{(}\PY{n}{state\PYZus{}input}\PY{p}{)}
        \PY{n}{l} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Dense}\PY{p}{(}\PY{l+m+mi}{64}\PY{p}{,} \PY{n}{activation}\PY{o}{=}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{relu}\PY{l+s+s1}{\PYZsq{}}\PY{p}{)}\PY{p}{(}\PY{n}{l}\PY{p}{)}
        \PY{n}{l} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Dense}\PY{p}{(}\PY{l+m+mi}{64}\PY{p}{,} \PY{n}{activation}\PY{o}{=}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{relu}\PY{l+s+s1}{\PYZsq{}}\PY{p}{)}\PY{p}{(}\PY{n}{l}\PY{p}{)}
        \PY{n}{net\PYZus{}out} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Dense}\PY{p}{(}\PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{action\PYZus{}size}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{,} \PY{n}{activation}\PY{o}{=}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{tanh}\PY{l+s+s1}{\PYZsq{}}\PY{p}{,}
                               \PY{n}{kernel\PYZus{}initializer}\PY{o}{=}\PY{n}{last\PYZus{}init}\PY{p}{)}\PY{p}{(}\PY{n}{l}\PY{p}{)}
        \PY{n}{net\PYZus{}out} \PY{o}{=} \PY{n}{net\PYZus{}out} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{upper\PYZus{}bound}
        \PY{n}{model} \PY{o}{=} \PY{n}{keras}\PY{o}{.}\PY{n}{Model}\PY{p}{(}\PY{n}{state\PYZus{}input}\PY{p}{,} \PY{n}{net\PYZus{}out}\PY{p}{)}
        \PY{n}{model}\PY{o}{.}\PY{n}{summary}\PY{p}{(}\PY{p}{)}
        \PY{k}{return} \PY{n}{model}
\end{Verbatim}


==> pygtex_files/actor_train-py.tex <==
\begin{Verbatim}[commandchars=\\\{\},baselinestretch=0.9,frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\tiny]
\PY{k}{class} \PY{n+nc}{PPOActor}\PY{p}{:}
    \PY{k}{def} \PY{n+nf}{train}\PY{p}{(}\PY{n+nb+bp}{self}\PY{p}{,} \PY{n}{state\PYZus{}batch}\PY{p}{,} \PY{n}{action\PYZus{}batch}\PY{p}{,} \PY{n}{advantages}\PY{p}{,} \PY{n}{old\PYZus{}pi}\PY{p}{)}\PY{p}{:}

        \PY{k}{with} \PY{n}{tf}\PY{o}{.}\PY{n}{GradientTape}\PY{p}{(}\PY{p}{)} \PY{k}{as} \PY{n}{tape}\PY{p}{:}
            \PY{n}{mean} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{squeeze}\PY{p}{(}\PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{model}\PY{p}{(}\PY{n}{state\PYZus{}batch}\PY{p}{)}\PY{p}{)}
            \PY{n}{std} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{squeeze}\PY{p}{(}\PY{n}{tf}\PY{o}{.}\PY{n}{exp}\PY{p}{(}\PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{model}\PY{o}{.}\PY{n}{logstd}\PY{p}{)}\PY{p}{)}
            \PY{n}{pi} \PY{o}{=} \PY{n}{tfp}\PY{o}{.}\PY{n}{distributions}\PY{o}{.}\PY{n}{Normal}\PY{p}{(}\PY{n}{mean}\PY{p}{,} \PY{n}{std}\PY{p}{)}
            \PY{n}{ratio} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{exp}\PY{p}{(}\PY{n}{pi}\PY{o}{.}\PY{n}{log\PYZus{}prob}\PY{p}{(}\PY{n}{tf}\PY{o}{.}\PY{n}{squeeze}\PY{p}{(}\PY{n}{action\PYZus{}batch}\PY{p}{)}\PY{p}{)} \PY{o}{\PYZhy{}}
                           \PY{n}{old\PYZus{}pi}\PY{o}{.}\PY{n}{log\PYZus{}prob}\PY{p}{(}\PY{n}{tf}\PY{o}{.}\PY{n}{squeeze}\PY{p}{(}\PY{n}{action\PYZus{}batch}\PY{p}{)}\PY{p}{)}\PY{p}{)}
            \PY{n}{surr} \PY{o}{=} \PY{n}{ratio} \PY{o}{*} \PY{n}{advantages}  \PY{c+c1}{\PYZsh{} surrogate function}
            \PY{n}{kl} \PY{o}{=} \PY{n}{tfp}\PY{o}{.}\PY{n}{distributions}\PY{o}{.}\PY{n}{kl\PYZus{}divergence}\PY{p}{(}\PY{n}{old\PYZus{}pi}\PY{p}{,} \PY{n}{pi}\PY{p}{)}
            \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{kl\PYZus{}value} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{reduce\PYZus{}mean}\PY{p}{(}\PY{n}{kl}\PY{p}{)}
            \PY{k}{if} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{method} \PY{o}{==} \PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{penalty}\PY{l+s+s1}{\PYZsq{}}\PY{p}{:}  \PY{c+c1}{\PYZsh{} ppo\PYZhy{}penalty method}
                \PY{n}{actor\PYZus{}loss} \PY{o}{=} \PY{o}{\PYZhy{}}\PY{p}{(}\PY{n}{tf}\PY{o}{.}\PY{n}{reduce\PYZus{}mean}\PY{p}{(}\PY{n}{surr} \PY{o}{\PYZhy{}} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{lam} \PY{o}{*} \PY{n}{kl}\PY{p}{)}\PY{p}{)}
                \PY{c+c1}{\PYZsh{} self.update\PYZus{}lambda()}
            \PY{k}{elif} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{method} \PY{o}{==} \PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{clip}\PY{l+s+s1}{\PYZsq{}}\PY{p}{:}  \PY{c+c1}{\PYZsh{} ppo\PYZhy{}clip method}
                \PY{n}{actor\PYZus{}loss} \PY{o}{=} \PY{o}{\PYZhy{}} \PY{n}{tf}\PY{o}{.}\PY{n}{reduce\PYZus{}mean}\PY{p}{(}
                    \PY{n}{tf}\PY{o}{.}\PY{n}{minimum}\PY{p}{(}\PY{n}{surr}\PY{p}{,} \PY{n}{tf}\PY{o}{.}\PY{n}{clip\PYZus{}by\PYZus{}value}\PY{p}{(}\PY{n}{ratio}\PY{p}{,}
                                                      \PY{l+m+mf}{1.} \PY{o}{\PYZhy{}} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{epsilon}\PY{p}{,} \PY{l+m+mf}{1.} \PY{o}{+} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{epsilon}\PY{p}{)} \PY{o}{*} \PY{n}{advantages}\PY{p}{)}\PY{p}{)}
            \PY{n}{actor\PYZus{}weights} \PY{o}{=} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{model}\PY{o}{.}\PY{n}{trainable\PYZus{}variables}

        \PY{c+c1}{\PYZsh{} outside gradient tape}
        \PY{n}{actor\PYZus{}grad} \PY{o}{=} \PY{n}{tape}\PY{o}{.}\PY{n}{gradient}\PY{p}{(}\PY{n}{actor\PYZus{}loss}\PY{p}{,} \PY{n}{actor\PYZus{}weights}\PY{p}{)}
        \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{optimizer}\PY{o}{.}\PY{n}{apply\PYZus{}gradients}\PY{p}{(}\PY{n+nb}{zip}\PY{p}{(}\PY{n}{actor\PYZus{}grad}\PY{p}{,} \PY{n}{actor\PYZus{}weights}\PY{p}{)}\PY{p}{)}

        \PY{k}{return} \PY{n}{actor\PYZus{}loss}\PY{o}{.}\PY{n}{numpy}\PY{p}{(}\PY{p}{)}\PY{p}{,} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{kl\PYZus{}value}\PY{o}{.}\PY{n}{numpy}\PY{p}{(}\PY{p}{)}

    \PY{k}{def} \PY{n+nf}{update\PYZus{}lambda}\PY{p}{(}\PY{n+nb+bp}{self}\PY{p}{)}\PY{p}{:}
        \PY{c+c1}{\PYZsh{} update the lambda value after each epoch}
        \PY{k}{if} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{kl\PYZus{}value} \PY{o}{\PYZlt{}} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{kl\PYZus{}target} \PY{o}{/} \PY{l+m+mf}{1.5}\PY{p}{:}
            \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{lam} \PY{o}{/}\PY{o}{=} \PY{l+m+mi}{2}
        \PY{k}{elif} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{kl\PYZus{}value} \PY{o}{\PYZgt{}} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{kl\PYZus{}target} \PY{o}{*} \PY{l+m+mf}{1.5}\PY{p}{:}
            \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{lam} \PY{o}{*}\PY{o}{=} \PY{l+m+mi}{2}
    
\end{Verbatim}


==> pygtex_files/agent_train-py.tex <==
\begin{Verbatim}[commandchars=\\\{\},baselinestretch=0.9,frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\tiny]
\PY{k}{def} \PY{n+nf}{train}\PY{p}{(}\PY{n+nb+bp}{self}\PY{p}{,} \PY{n}{states}\PY{p}{,} \PY{n}{actions}\PY{p}{,} \PY{n}{rewards}\PY{p}{,} \PY{n}{next\PYZus{}states}\PY{p}{,} \PY{n}{dones}\PY{p}{,} \PY{n}{epochs}\PY{o}{=}\PY{l+m+mi}{20}\PY{p}{)}\PY{p}{:}

        \PY{n}{states} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{convert\PYZus{}to\PYZus{}tensor}\PY{p}{(}\PY{n}{states}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n}{tf}\PY{o}{.}\PY{n}{float32}\PY{p}{)}
        \PY{n}{next\PYZus{}states} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{convert\PYZus{}to\PYZus{}tensor}\PY{p}{(}\PY{n}{next\PYZus{}states}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n}{tf}\PY{o}{.}\PY{n}{float32}\PY{p}{)}
        \PY{n}{actions} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{convert\PYZus{}to\PYZus{}tensor}\PY{p}{(}\PY{n}{actions}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n}{tf}\PY{o}{.}\PY{n}{float32}\PY{p}{)}
        \PY{n}{rewards} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{convert\PYZus{}to\PYZus{}tensor}\PY{p}{(}\PY{n}{rewards}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n}{tf}\PY{o}{.}\PY{n}{float32}\PY{p}{)}
        \PY{n}{dones} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{convert\PYZus{}to\PYZus{}tensor}\PY{p}{(}\PY{n}{dones}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n}{tf}\PY{o}{.}\PY{n}{float32}\PY{p}{)}

        \PY{c+c1}{\PYZsh{} compute advantages and discounted cumulative rewards}
        \PY{n}{target\PYZus{}values}\PY{p}{,} \PY{n}{advantages} \PY{o}{=} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{compute\PYZus{}advantages}\PY{p}{(}\PY{n}{states}\PY{p}{,} \PY{n}{next\PYZus{}states}\PY{p}{,} \PY{n}{rewards}\PY{p}{,} \PY{n}{dones}\PY{p}{)}

        \PY{n}{target\PYZus{}values} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{convert\PYZus{}to\PYZus{}tensor}\PY{p}{(}\PY{n}{target\PYZus{}values}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n}{tf}\PY{o}{.}\PY{n}{float32}\PY{p}{)}
        \PY{n}{advantages} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{convert\PYZus{}to\PYZus{}tensor}\PY{p}{(}\PY{n}{advantages}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n}{tf}\PY{o}{.}\PY{n}{float32}\PY{p}{)}

        \PY{c+c1}{\PYZsh{} current action probability distribution}
        \PY{n}{mean}\PY{p}{,} \PY{n}{std} \PY{o}{=} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{actor}\PY{p}{(}\PY{n}{states}\PY{p}{)}
        \PY{n}{pi} \PY{o}{=} \PY{n}{tfp}\PY{o}{.}\PY{n}{distributions}\PY{o}{.}\PY{n}{Normal}\PY{p}{(}\PY{n}{mean}\PY{p}{,} \PY{n}{std}\PY{p}{)}

        \PY{n}{n\PYZus{}split} \PY{o}{=} \PY{n+nb}{len}\PY{p}{(}\PY{n}{rewards}\PY{p}{)} \PY{o}{/}\PY{o}{/} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}
        \PY{k}{assert} \PY{n}{n\PYZus{}split} \PY{o}{\PYZgt{}} \PY{l+m+mi}{0}\PY{p}{,} \PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{there should be at least one split}\PY{l+s+s1}{\PYZsq{}}

        \PY{n}{indexes} \PY{o}{=} \PY{n}{np}\PY{o}{.}\PY{n}{arange}\PY{p}{(}\PY{n}{n\PYZus{}split}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n+nb}{int}\PY{p}{)}

        \PY{c+c1}{\PYZsh{} training}
        \PY{n}{a\PYZus{}loss\PYZus{}list} \PY{o}{=} \PY{p}{[}\PY{p}{]}
        \PY{n}{c\PYZus{}loss\PYZus{}list} \PY{o}{=} \PY{p}{[}\PY{p}{]}
        \PY{n}{kl\PYZus{}list} \PY{o}{=} \PY{p}{[}\PY{p}{]}
        \PY{n}{np}\PY{o}{.}\PY{n}{random}\PY{o}{.}\PY{n}{shuffle}\PY{p}{(}\PY{n}{indexes}\PY{p}{)}
        \PY{k}{for} \PY{n}{\PYZus{}} \PY{o+ow}{in} \PY{n+nb}{range}\PY{p}{(}\PY{n}{epochs}\PY{p}{)}\PY{p}{:}
            \PY{k}{for} \PY{n}{i} \PY{o+ow}{in} \PY{n}{indexes}\PY{p}{:}
                \PY{n}{old\PYZus{}pi} \PY{o}{=} \PY{n}{pi}\PY{p}{[}\PY{n}{i} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{:} \PY{p}{(}\PY{n}{i} \PY{o}{+} \PY{l+m+mi}{1}\PY{p}{)} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{]}
                \PY{n}{s\PYZus{}split} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{gather}\PY{p}{(}\PY{n}{states}\PY{p}{,} \PY{n}{indices}\PY{o}{=}\PY{n}{np}\PY{o}{.}\PY{n}{arange}\PY{p}{(}\PY{n}{i} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{,} \PY{p}{(}\PY{n}{i}\PY{o}{+}\PY{l+m+mi}{1}\PY{p}{)} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{)}\PY{p}{,} \PY{n}{axis}\PY{o}{=}\PY{l+m+mi}{0}\PY{p}{)}
                \PY{n}{a\PYZus{}split} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{gather}\PY{p}{(}\PY{n}{actions}\PY{p}{,} \PY{n}{indices}\PY{o}{=}\PY{n}{np}\PY{o}{.}\PY{n}{arange}\PY{p}{(}\PY{n}{i} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{,} \PY{p}{(}\PY{n}{i}\PY{o}{+}\PY{l+m+mi}{1}\PY{p}{)} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{)}\PY{p}{,} \PY{n}{axis}\PY{o}{=}\PY{l+m+mi}{0}\PY{p}{)}
                \PY{n}{tv\PYZus{}split} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{gather}\PY{p}{(}\PY{n}{target\PYZus{}values}\PY{p}{,} \PY{n}{indices}\PY{o}{=}\PY{n}{np}\PY{o}{.}\PY{n}{arange}\PY{p}{(}\PY{n}{i} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{,} \PY{p}{(}\PY{n}{i}\PY{o}{+}\PY{l+m+mi}{1}\PY{p}{)} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{)}\PY{p}{,} \PY{n}{axis}\PY{o}{=}\PY{l+m+mi}{0}\PY{p}{)}
                \PY{n}{adv\PYZus{}split} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{gather}\PY{p}{(}\PY{n}{advantages}\PY{p}{,} \PY{n}{indices}\PY{o}{=}\PY{n}{np}\PY{o}{.}\PY{n}{arange}\PY{p}{(}\PY{n}{i} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{,} \PY{p}{(}\PY{n}{i}\PY{o}{+}\PY{l+m+mi}{1}\PY{p}{)} \PY{o}{*} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{batch\PYZus{}size}\PY{p}{)}\PY{p}{,} \PY{n}{axis}\PY{o}{=}\PY{l+m+mi}{0}\PY{p}{)}

                \PY{c+c1}{\PYZsh{} update critic}
                \PY{n}{cl} \PY{o}{=} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{critic}\PY{o}{.}\PY{n}{train}\PY{p}{(}\PY{n}{s\PYZus{}split}\PY{p}{,} \PY{n}{tv\PYZus{}split}\PY{p}{)}
                \PY{n}{c\PYZus{}loss\PYZus{}list}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{n}{cl}\PY{p}{)}

                \PY{c+c1}{\PYZsh{} update actor}
                \PY{n}{a\PYZus{}loss\PYZus{}list}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{actor}\PY{o}{.}\PY{n}{train}\PY{p}{(}\PY{n}{s\PYZus{}split}\PY{p}{,} \PY{n}{a\PYZus{}split}\PY{p}{,}
                                                    \PY{n}{adv\PYZus{}split}\PY{p}{,} \PY{n}{old\PYZus{}pi}\PY{p}{,} \PY{n}{cl}\PY{p}{)}\PY{p}{)}
                \PY{n}{kl\PYZus{}list}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{actor}\PY{o}{.}\PY{n}{kl\PYZus{}value}\PY{p}{)}

            \PY{c+c1}{\PYZsh{} update lambda once in each epoch}
            \PY{c+c1}{\PYZsh{} if self.method == \PYZsq{}penalty\PYZsq{}:}
            \PY{c+c1}{\PYZsh{}     self.actor.update\PYZus{}beta()}

        \PY{n}{actor\PYZus{}loss} \PY{o}{=} \PY{n}{np}\PY{o}{.}\PY{n}{mean}\PY{p}{(}\PY{n}{a\PYZus{}loss\PYZus{}list}\PY{p}{)}
        \PY{n}{critic\PYZus{}loss} \PY{o}{=} \PY{n}{np}\PY{o}{.}\PY{n}{mean}\PY{p}{(}\PY{n}{c\PYZus{}loss\PYZus{}list}\PY{p}{)}
        \PY{n}{kld\PYZus{}mean} \PY{o}{=} \PY{n}{np}\PY{o}{.}\PY{n}{mean}\PY{p}{(}\PY{n}{kl\PYZus{}list}\PY{p}{)}

        \PY{k}{return} \PY{n}{actor\PYZus{}loss}\PY{p}{,} \PY{n}{critic\PYZus{}loss}\PY{p}{,} \PY{n}{kld\PYZus{}mean}
\end{Verbatim}


==> pygtex_files/critic_model-py.tex <==
\begin{Verbatim}[commandchars=\\\{\},baselinestretch=0.9,frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\tiny]
\PY{k}{class} \PY{n+nc}{PPOCritic}\PY{p}{:}
    \PY{k}{def} \PY{n+nf}{\PYZus{}build\PYZus{}net}\PY{p}{(}\PY{n+nb+bp}{self}\PY{p}{)}\PY{p}{:}
        \PY{n}{state\PYZus{}input} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Input}\PY{p}{(}\PY{n}{shape}\PY{o}{=}\PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{state\PYZus{}size}\PY{p}{)}
        \PY{n}{out} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Dense}\PY{p}{(}\PY{l+m+mi}{64}\PY{p}{,} \PY{n}{activation}\PY{o}{=}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{relu}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}\PY{p}{(}\PY{n}{state\PYZus{}input}\PY{p}{)}
        \PY{n}{out} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Dense}\PY{p}{(}\PY{l+m+mi}{64}\PY{p}{,} \PY{n}{activation}\PY{o}{=}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{relu}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}\PY{p}{(}\PY{n}{out}\PY{p}{)}
        \PY{n}{out} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Dense}\PY{p}{(}\PY{l+m+mi}{64}\PY{p}{,} \PY{n}{activation}\PY{o}{=}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{relu}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}\PY{p}{(}\PY{n}{out}\PY{p}{)}
        \PY{n}{net\PYZus{}out} \PY{o}{=} \PY{n}{layers}\PY{o}{.}\PY{n}{Dense}\PY{p}{(}\PY{l+m+mi}{1}\PY{p}{)}\PY{p}{(}\PY{n}{out}\PY{p}{)}

        \PY{c+c1}{\PYZsh{} Outputs single value for give state\PYZhy{}action}
        \PY{n}{model} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{keras}\PY{o}{.}\PY{n}{Model}\PY{p}{(}\PY{n}{inputs}\PY{o}{=}\PY{n}{state\PYZus{}input}\PY{p}{,} \PY{n}{outputs}\PY{o}{=}\PY{n}{net\PYZus{}out}\PY{p}{)}
        \PY{n}{model}\PY{o}{.}\PY{n}{summary}\PY{p}{(}\PY{p}{)}
        \PY{k}{return} \PY{n}{model}
\end{Verbatim}


==> pygtex_files/critic_train-py.tex <==
\begin{Verbatim}[commandchars=\\\{\},baselinestretch=0.9,frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\tiny]
\PY{k}{class} \PY{n+nc}{PPOCritic}\PY{p}{:}
    \PY{k}{def} \PY{n+nf}{train}\PY{p}{(}\PY{n+nb+bp}{self}\PY{p}{,} \PY{n}{state\PYZus{}batch}\PY{p}{,} \PY{n}{disc\PYZus{}rewards}\PY{p}{)}\PY{p}{:}
        \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{train\PYZus{}step\PYZus{}count} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
        \PY{k}{with} \PY{n}{tf}\PY{o}{.}\PY{n}{GradientTape}\PY{p}{(}\PY{p}{)} \PY{k}{as} \PY{n}{tape}\PY{p}{:}
            \PY{n}{critic\PYZus{}weights} \PY{o}{=} \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{model}\PY{o}{.}\PY{n}{trainable\PYZus{}variables}
            \PY{n}{critic\PYZus{}value} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{squeeze}\PY{p}{(}\PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{model}\PY{p}{(}\PY{n}{state\PYZus{}batch}\PY{p}{)}\PY{p}{)}
            \PY{n}{critic\PYZus{}loss} \PY{o}{=} \PY{n}{tf}\PY{o}{.}\PY{n}{math}\PY{o}{.}\PY{n}{reduce\PYZus{}mean}\PY{p}{(}\PY{n}{tf}\PY{o}{.}\PY{n}{square}\PY{p}{(}\PY{n}{disc\PYZus{}rewards} \PY{o}{\PYZhy{}} \PY{n}{critic\PYZus{}value}\PY{p}{)}\PY{p}{)}
        \PY{n}{critic\PYZus{}grad} \PY{o}{=} \PY{n}{tape}\PY{o}{.}\PY{n}{gradient}\PY{p}{(}\PY{n}{critic\PYZus{}loss}\PY{p}{,} \PY{n}{critic\PYZus{}weights}\PY{p}{)}
        \PY{n+nb+bp}{self}\PY{o}{.}\PY{n}{optimizer}\PY{o}{.}\PY{n}{apply\PYZus{}gradients}\PY{p}{(}\PY{n+nb}{zip}\PY{p}{(}\PY{n}{critic\PYZus{}grad}\PY{p}{,} \PY{n}{critic\PYZus{}weights}\PY{p}{)}\PY{p}{)}
        \PY{k}{return} \PY{n}{critic\PYZus{}loss}\PY{o}{.}\PY{n}{numpy}\PY{p}{(}\PY{p}{)}
\end{Verbatim}


==> pygtex_files/funcs-py.tex <==
\begin{Verbatim}[commandchars=\\\{\},frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\tiny]
\PY{k}{def} \PY{n+nf}{collect\PYZus{}trajectories}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{k}{pass}

\PY{k}{def} \PY{n+nf}{main}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{n}{scores\PYZus{}window} \PY{o}{=} \PY{n}{deque}\PY{p}{(}\PY{n}{maxlen}\PY{o}{=}\PY{l+m+mi}{100}\PY{p}{)}
    \PY{n}{save\PYZus{}scores} \PY{o}{=} \PY{p}{[}\PY{p}{]}
    \PY{k}{for} \PY{n}{s} \PY{o+ow}{in} \PY{n+nb}{range}\PY{p}{(}\PY{n}{max\PYZus{}seasons}\PY{p}{)}\PY{p}{:}
        \PY{c+c1}{\PYZsh{} collect trajectories}
        \PY{n}{states}\PY{p}{,} \PY{n}{actions}\PY{p}{,} \PY{n}{rewards}\PY{p}{,} \PY{n}{next\PYZus{}states}\PY{p}{,} \PY{n}{dones}\PY{p}{,} \PY{n}{ep\PYZus{}count} \PY{o}{=} \PYZbs{}
            \PY{n}{collect\PYZus{}trajectories}\PY{p}{(}\PY{n}{env}\PY{p}{,} \PY{n}{agent}\PY{p}{,} \PY{n}{tmax}\PY{o}{=}\PY{l+m+mi}{1000}\PY{p}{)}

        \PY{c+c1}{\PYZsh{} train the agent}
        \PY{n}{a\PYZus{}loss}\PY{p}{,} \PY{n}{c\PYZus{}loss}\PY{p}{,} \PY{n}{kld\PYZus{}value} \PY{o}{=} \PY{n}{agent}\PY{o}{.}\PY{n}{train}\PY{p}{(}\PY{n}{states}\PY{p}{,} \PY{n}{actions}\PY{p}{,} \PY{n}{rewards}\PY{p}{,}
                                                \PY{n}{next\PYZus{}states}\PY{p}{,} \PY{n}{dones}\PY{p}{,} \PY{n}{epochs}\PY{o}{=}\PY{l+m+mi}{10}\PY{p}{)}

        \PY{c+c1}{\PYZsh{} decay the clipping parameter over time}
        \PY{n}{agent}\PY{o}{.}\PY{n}{actor}\PY{o}{.}\PY{n}{epsilon} \PY{o}{*}\PY{o}{=} \PY{l+m+mf}{0.999}
        \PY{n}{agent}\PY{o}{.}\PY{n}{entropy\PYZus{}coeff} \PY{o}{*}\PY{o}{=} \PY{l+m+mf}{0.998}

        \PY{n}{season\PYZus{}score} \PY{o}{=} \PY{n}{np}\PY{o}{.}\PY{n}{sum}\PY{p}{(}\PY{n}{rewards}\PY{p}{,} \PY{n}{axis}\PY{o}{=}\PY{l+m+mi}{0}\PY{p}{)}
        \PY{n}{scores\PYZus{}window}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{n}{season\PYZus{}score}\PY{p}{)}
        \PY{n}{save\PYZus{}scores}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{n}{season\PYZus{}score}\PY{p}{)}
        \PY{n}{mean\PYZus{}reward} \PY{o}{=} \PY{n}{np}\PY{o}{.}\PY{n}{mean}\PY{p}{(}\PY{n}{scores\PYZus{}window}\PY{p}{)}

        \PY{k}{if} \PY{n}{best\PYZus{}score} \PY{o}{\PYZlt{}} \PY{n}{mean\PYZus{}reward}\PY{p}{:}
            \PY{n}{best\PYZus{}score} \PY{o}{=} \PY{n}{mean\PYZus{}reward}
            \PY{n}{agent}\PY{o}{.}\PY{n}{save\PYZus{}model}\PY{p}{(}\PY{n}{path}\PY{p}{,} \PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{actor\PYZus{}weights.h5}\PY{l+s+s1}{\PYZsq{}}\PY{p}{,} \PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{critic\PYZus{}weights.h5}\PY{l+s+s1}{\PYZsq{}}\PY{p}{)}
            \PY{k}{print}\PY{p}{(}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{*** Season:\PYZob{}\PYZcb{}, best score: \PYZob{}\PYZcb{}. Model Saved ***}\PY{l+s+s1}{\PYZsq{}}\PY{o}{.}\PY{n}{format}\PY{p}{(}\PY{n}{s}\PY{p}{,} \PY{n}{best\PYZus{}score}\PY{p}{)}\PY{p}{)}


        \PY{k}{if} \PY{n}{s} \PY{o}{\PYZgt{}} \PY{l+m+mi}{25} \PY{o+ow}{and} \PY{n}{best\PYZus{}score} \PY{o}{\PYZgt{}} \PY{l+m+mi}{50}\PY{p}{:}
            \PY{k}{print}\PY{p}{(}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{Problem is solved in \PYZob{}\PYZcb{} seasons.}\PY{l+s+s1}{\PYZsq{}}\PY{o}{.}\PY{n}{format}\PY{p}{(}\PY{n}{s}\PY{p}{)}\PY{p}{)}
            \PY{n}{agent}\PY{o}{.}\PY{n}{save\PYZus{}model}\PY{p}{(}\PY{n}{path}\PY{p}{,} \PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{actor\PYZus{}weights.h5}\PY{l+s+s1}{\PYZsq{}}\PY{p}{,} \PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{critic\PYZus{}weights.h5}\PY{l+s+s1}{\PYZsq{}}\PY{p}{)}
            \PY{k}{break}
    \PY{n}{env}\PY{o}{.}\PY{n}{close}\PY{p}{(}\PY{p}{)}
\end{Verbatim}


==> pygtex_files/test-py.tex <==
\begin{Verbatim}[commandchars=\\\{\},baselinestretch=0.9,frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\tiny]
\PY{c+c1}{\PYZsh{} Test the model}
\PY{k}{def} \PY{n+nf}{test}\PY{p}{(}\PY{n}{env}\PY{p}{,} \PY{n}{agent}\PY{p}{,} \PY{n}{path}\PY{o}{=}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{./}\PY{l+s+s1}{\PYZsq{}}\PY{p}{,} \PY{n}{max\PYZus{}eps}\PY{o}{=}\PY{l+m+mi}{10}\PY{p}{)}\PY{p}{:}
    \PY{n}{agent}\PY{o}{.}\PY{n}{load\PYZus{}model}\PY{p}{(}\PY{n}{path}\PY{p}{,} \PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{actor\PYZus{}weights.h5}\PY{l+s+s1}{\PYZsq{}}\PY{p}{,} \PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{critic\PYZus{}weights.h5}\PY{l+s+s1}{\PYZsq{}}\PY{p}{)}
    \PY{n}{ep\PYZus{}reward\PYZus{}list} \PY{o}{=} \PY{p}{[}\PY{p}{]}
    \PY{k}{for} \PY{n}{ep} \PY{o+ow}{in} \PY{n+nb}{range}\PY{p}{(}\PY{n}{max\PYZus{}eps}\PY{p}{)}\PY{p}{:}
        \PY{n}{obsv} \PY{o}{=} \PY{n}{env}\PY{o}{.}\PY{n}{reset}\PY{p}{(}\PY{p}{)}
        \PY{n}{state} \PY{o}{=} \PY{n}{np}\PY{o}{.}\PY{n}{asarray}\PY{p}{(}\PY{n}{obsv}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n}{np}\PY{o}{.}\PY{n}{float32}\PY{p}{)} \PY{o}{/} \PY{l+m+mf}{255.0}  
        \PY{n}{ep\PYZus{}reward} \PY{o}{=} \PY{l+m+mi}{0}
        \PY{n}{t} \PY{o}{=} \PY{l+m+mi}{0}
        \PY{k}{while} \PY{n+nb+bp}{True}\PY{p}{:}
            \PY{n}{env}\PY{o}{.}\PY{n}{render}\PY{p}{(}\PY{p}{)}        \PY{c+c1}{\PYZsh{} show animation}
            \PY{n}{action} \PY{o}{=} \PY{n}{agent}\PY{o}{.}\PY{n}{policy}\PY{p}{(}\PY{n}{state}\PY{p}{)}
            \PY{n}{next\PYZus{}obsv}\PY{p}{,} \PY{n}{reward}\PY{p}{,} \PY{n}{done}\PY{p}{,} \PY{n}{\PYZus{}} \PY{o}{=} \PY{n}{env}\PY{o}{.}\PY{n}{step}\PY{p}{(}\PY{n}{action}\PY{p}{)}
            \PY{n}{next\PYZus{}state} \PY{o}{=} \PY{n}{np}\PY{o}{.}\PY{n}{asarray}\PY{p}{(}\PY{n}{next\PYZus{}obsv}\PY{p}{,} \PY{n}{dtype}\PY{o}{=}\PY{n}{np}\PY{o}{.}\PY{n}{float32}\PY{p}{)} \PY{o}{/} \PY{l+m+mf}{255.0}  
            \PY{n}{ep\PYZus{}reward} \PY{o}{+}\PY{o}{=} \PY{n}{reward}
            \PY{n}{t} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
            \PY{n}{state} \PY{o}{=} \PY{n}{next\PYZus{}state}
            \PY{k}{if} \PY{n}{done}\PY{p}{:}
                \PY{n}{ep\PYZus{}reward\PYZus{}list}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{n}{ep\PYZus{}reward}\PY{p}{)}
                \PY{k}{print}\PY{p}{(}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{Episode:\PYZob{}\PYZcb{}, Reward:\PYZob{}\PYZcb{}}\PY{l+s+s1}{\PYZsq{}}\PY{o}{.}\PY{n}{format}\PY{p}{(}\PY{n}{ep}\PY{p}{,} \PY{n}{ep\PYZus{}reward}\PY{p}{)}\PY{p}{)}
                \PY{k}{break}

    \PY{k}{print}\PY{p}{(}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{Avg Episodic Reward: }\PY{l+s+s1}{\PYZsq{}}\PY{p}{,} \PY{n}{np}\PY{o}{.}\PY{n}{mean}\PY{p}{(}\PY{n}{ep\PYZus{}reward\PYZus{}list}\PY{p}{)}\PY{p}{)}
    \PY{n}{env}\PY{o}{.}\PY{n}{close}\PY{p}{(}\PY{p}{)}
\end{Verbatim}

